Sharing LRU Cache Resources among Content Providers: A Utility-Based Approach

In this paper, we consider the problem of allocating cache resources among multiple content providers. The cache can be partitioned into slices and each partition can be dedicated to a particular content provider, or shared among a number of them. It is assumed that each partition employs the LRU policy for managing content. We propose utility-driven partitioning, where we associate with each content provider a utility that is a function of the hit rate observed by the content provider. We consider two scenarios: i)~content providers serve disjoint sets of files, ii)~there is some overlap in the content served by multiple content providers. In the first case, we prove that cache partitioning outperforms cache sharing as cache size and numbers of contents served by providers go to infinity. In the second case, It can be beneficial to have separate partitions for overlapped content. In the case of two providers, it is usually always beneficial to allocate a cache partition to serve all overlapped content and separate partitions to serve the non-overlapped contents of both providers. We establish conditions when this is true asymptotically but also present an example where it is not true asymptotically. We develop online algorithms that dynamically adjust partition sizes in order to maximize the overall utility and prove that they converge to optimal solutions, and through numerical evaluations, we show they are effective.

==> introduction-old.tex <==
\section{Introdcution}
The increase in data traffic over the past years is predicted to continue more aggressively, with the global Internet traffic in 2019 estimated to reach 64 times of its entire volume in 2005~\cite{cisco14}.
The growth in data traffic is recognized to be due to streaming of video on-demand content over cellular networks.
However, traditional methods such as increasing the amount of spectrum or deploying more base stations are not sufficient to cope with the predicted traffic increase~\cite{Andrews12, Golrezaei12}. Caching is recognized, in current and future Internet architecture proposals, as one of the most effective means to improve the performance of web applications.
By bringing the content closer to the users, caches greatly reduce network bandwidth usage, load on servers, and the service delay perceived by the end-users~\cite{borst10}.

Internet is becoming an increasingly heterogeneous environment as more and more devices with diverse technologies join the network, creating new content producers and consumers. Different types of applications vary in traffic characteristics and quality of service requirements. Such an increasing diversity in service expectations advocates the need for content delivery infrastructures with service differentiation among different applications and content classes. Moreover, service providers may have different contracts with different content providers to provide them with a better service for a negotiated price. This requires the caching system to distinguish between different content providers. How to effectively share limited resources between different types of traffic, while at the same time having the ability to provide differentiated services, becomes an urgent task that needs to be addressed~\cite{Zhang13}.

Static and dynamic partitioning of the cache space has been proposed by researchers~\cite{lu04, Carofiglio11}, in order to provide differentiated caching services from a shared storage system. In this paper, we propose a utility-driven cache partitioning framework, where each content provider has an associated utility and the cache space is partitioned and managed so as to maximize the aggregate utility for all content providers. Utilities represent the trade-off of a content provider's satisfaction and cost of storing content in the cache. Our framework allows us to develop \emph{online} algorithms for cache management that we prove achieve optimal performance. Our framework also has implications for distributed pricing and control mechanisms and hence is well-suited for designing cache market economic models.

Our main contributions in this paper can be summarized as follows:
\begin{itemize}[leftmargin=*]
\item We formulate a utility--based optimization framework for maximizing content providers' utility subject to cache capacity constraints at the service provider. We derive optimal partitions for two possible cases: 1) content providers serve completely distinct sets of contents, 2) some contents are served by multiple content providers.

\item We develop online algorithms for managing cache partitions, and prove the convergence of these algorithms to the optimal solution using Lyapunov functions.

\item We show that our framework can be used in revenue based models where content providers react to prices set by (cache) service providers without revealing their utility functions.

\item We perform simulations to show the efficiency of our online algorithms using different utility functions with different fairness implications.
\end{itemize}

The remainder of this paper is organized as follows. We review related work in the next section. Section~\ref{sec:model} explains the network model considered in this paper, and Section~\ref{sec:problem} describes our approach in constructing utility--maximizing cache partitions. In Section~\ref{sec:online}, we develop online algorithms for implementing utility--maximizing cache partitioning. We present simulation results in Section~\ref{sec:simulation}, and discuss prospects and implications of our utility--maximization framework in Section~\ref{sec:discussion}. Finally, we conclude the paper in Section~\ref{sec:conclusion}.

==> model_old.tex <==
\section{Problem Setting \& Basic Model}
\label{sec:model}
\begin{figure}[t]
\centering
  	\includegraphics[scale=0.24]{sc_model2.png}
\caption{Network Model.}
 %\vspace{-0.5cm}
    \label{fig:model}
\end{figure}

Consider a network as shown in Figure~\ref{fig:model}, where users access content, \eg~videos,  from $K$ content providers (CPs).
CP $k~(k=1,\ldots,K)$ serves a set $F_k$ of unit size files and all CPs share a content cache, supplied by a third-party network provider, referred to as a cache manager hereafter.
% is deployed in the network to enhance content delivery to the users. 
%One example of such a network could be users streaming video from content providers such as YouTube, Netflix or Amazon Video. 
Content providers have business relations with the cache manager and pay for cache resources. 
%The cache manager needs to allocate the cache storage resources to the CPs either to maximize the cache utilization or to maximize the {\em utilities} of CPs (thus its own profit).
There are two possible scenarios: i)~the content objects offered by the CPs are all {\em distinct}; and ii)~some {\em common} objects are provided by different CPs. Due to disparate user bases, the access patterns of these content objects may vary across the CPs.
% in the best way possible to keep the content providers satisfied, so that its profit is maximized. 
%Two cases arise depending on whether content providers serve completely separate content, or if there exist content that is served by multiple content %providers. If content providers only serve the content they produce/own, the set of content served by content providers can be assumed to be distinct. If content providers also serve content from other producers, some content can be served by multiple content providers.
Our goal in this paper is to study the {\em cache allocation problem}  for a single network cache element, where the cache manager aims to
maximize the overall cache utilization or  the weighted sum of the utilities of the content providers so as to maximize its own profit.
% (see Section~\ref{sec:model} for discussion on the implication of our work on network economic modeling of cache services for ICNs).

We assume that requests are described by a Poisson process with request rate for file $i$ of CP $k$ being ${\lambda_{ik}, i\in F_k, k = 1,\ldots,K}$. Associated with each CP is a utility $U_k(h_k)$ that is a {\em strictly increasing, concave} function of the hit rate $h_k$ over all its files. In its most general form, the cache manager wishes to maximize a {\em weighted} sum of the utilities over all content providers, $\sum_{k}{w_k U_k(h_k)}$, through a proper allocation of cache space to the CPs. The weights $w_k$ are chosen by the cache manager to reflect business preferences such as financial incentives or legal obligations. In the simple case where $w_k=1$ and $U_k(h_k)=h_k$, the objective becomes that of maximizing the overall cache hit rate, which provides a measure of  the overall cache utilization efficiency.

\vspace*{2pt}
\noindent
{\bf Sharing or Partitioning? That is the Question!}
The cache manager can either i)  have CPs {\em share} the cache where the content objects offered by all CPs compete for the storage space based on their access patterns, or ii) partition the cache into (virtual) slices and allocate one slice to each CP (or share some slices among  certain (subsets of) CPs), thereby restricting cache contention to the set of content objects owned by one CP (or certain subset of CPs). 
The cache is assumed to have capacity for $C$ files in total. Let $P$ denote the number of partitions and let $\mathbf{C} = (C_1, C_2, \ldots, C_P)$ denote the vector of partition sizes. For each content provider $k$, hit rate is a function of the partition sizes $h_k(\mathbf{C})$. The problem of utility-based cache resource allocation can then be formulated as follows:
\begin{align*}
\label{eq:main}
\text{maximize} \quad &\sum_{k=1}^{K}{w_kU_k\Big(h_k(\mathbf{C})\Big)} \notag\\
\text{such that} \quad &\sum_{p=1}^{P}{C_p} \le C \\
& C_p = 0, 1, 2,\ldots; \quad p=1, 2, \ldots, P. \notag
\end{align*}

Note that the above formulation is an integer programming problem that is typically hard to solve. However, in practice caches are large and therefore we assume $C_p$ can take any real value, as the rounding error will be negligible.

To determine the number of slices and that what files should be requested from which partition, the cache manager proceeds as follows. Files are first grouped into disjoint sets according to which content providers serve them. The cache manager then decides how many partitions to create, and whether to dedicate a separate partition for each set of files, or have multiple sets share a partition. In the next section, we explain what could change if the cache manager made partitioning decisions on a per file basis rather than sets of files.


%\subsection{Cache Characteristic Time}
%\label{sec:che}
\vspace*{2pt}
\noindent
{\bf Cache Characteristic Time.}
Che~\etal~\cite{Che01} introduced the notion of \emph{cache characteristic time} and used it to approximate the hit probability of an LRU cache with Poisson arrivals. According to Che~\etal~\cite{Che01} the hit probability of a file with request rate $\lambda_i$ in an LRU cache can be approximated by
\[o(\lambda_i, T) = 1 - e^{-\lambda_iT},\]
where $\lambda_i$ is the request rate for file $i$, and $T$ is a constant denoting the {\em characteristic time} of the LRU cache with size $C$.

The characteristic time approximation has been theoretically justified and shown to be accurate in practice~\cite{Fricker12}. This notion has been generalized to a wider range of caching policies, \eg\ FIFO and Random, and more general arrival processes~\cite{Michelle14}. For a caching policy that can be modeled using a characteristic time, we use $o\Big(\lambda_i,T(C)\Big)$ to denote the hit probability of file $i$ where $T(C)$ denotes the characteristic time as a function of the cache size. $T(C)$ is computed as the unique solution to the equation
\[\sum_{i=1}^N{o\Big(\lambda_i,T(C)\Big)} = C,\]
where $N$ is the number of files accessing the cache. According to the above calculations, cache hit rate is expressed as
\[h(C) = \sum_{i=1}^N{\lambda_io\Big(\lambda_i,T(C)\Big)}.\]

In this paper, we consider caching policies that can be modeled using this characteristic time approximation. We further assume that the hit rate $h(C)$ is a concave and increasing function of the cache size. It is easy to see (as we show in~\cite{supplement}) that this assumption holds for policies such as LRU, FIFO and Random.

%Note that the concavity of $h(C)$ is not a strong assumption. 


==> problem_old.tex <==
\section{Cache Resource Allocation among Multiple Content Providers}
\label{sec:problem}
In this section, we formulate cache management as a utility maximization problem. We introduce two formulations, one for the case where content providers serve distinct contents, and another one for the case where some contents are served by multiple providers.

\subsection{Content Providers with Distinct Objects}
The first question one needs to answer in formulating this problem is
whether to partition the cache or share it among all content
providers.  If partitioning yields the best strategy, then the second
question is how the cache should be partitioned.

The following theorem answers this question:
\begin{theorem}
\label{thm:distinct_partition}
With $K$ content providers serving distinct contents, the LRU cache should be partitioned into $K$ slices.
\end{theorem}
\begin{proof}
See Appendix~\ref{sec:proof_partition}.
\end{proof}

%A direct consequence of the above theorem is that
%\begin{corollary}
%With $K$ content providers serving distinct contents, the LRU cache should be partitioned into $K$ slices.
%\end{corollary}
%\begin{proof}
%See Appendix~\ref{sec:proof_k_partitions}.
%\end{proof}

Based on the above theorem, we can now formulate the utility--maximizing resource allocation problem for content providers with distinct files as follows:
\begin{align}
\label{eq:opt}
\text{maximize} \quad &\sum_{k=1}^{K}{w_k U_k\Big(h_k(C_k)\Big)} \notag\\
\text{such that} \quad &\sum_{k=1}^{K}{C_k} \le C \\
& C_k \ge 0, \quad k=1, 2, \ldots, K. \notag
\end{align}

In our formulation, we assume that each partition employs the LRU policy for managing the cache content. Therefore, we can adopt the concept of \emph{characteristic time} for each partition to compute the average hit rate for a content provider as
\[h_k(C_k) = \sum_{i\in F_k}{\lambda_{ik}(1 - e^{-\lambda_{ik}T_k})},\]
where $T_k$ denotes the characteristic time of the partition with size $C_k$ dedicated to content provider $k$. $T_k$ is the unique solution to the equation
\[\sum_{i\in F_k}{(1 - e^{-\lambda_{ik}T_k})} = C_k.\]

Note that our assumption that files have a unit size implies that the capacity of a cache (partition) would be determined in terms of the number of files it can hold, \ie\ $C_k$ is an integer. However, since in practice caches are large, we assume $C_k$s can take real values, as the rounding error will be negligible. Therefore, we do not consider optimization problem~\eqref{eq:opt} as an integer programming problem that is hard to solve. Rather, we assume that the optimal solution can be found in polynomial time. The following theorem establishes that the resource allocation problem~\eqref{eq:opt} has a unique optimal solution:
\begin{theorem}
\label{thrm:opt_exists}
Resource allocation problem~\eqref{eq:opt} has a unique optimal solution.
\end{theorem}

\begin{proof}
In Appendix~\ref{sec:proof_obj}, objective function of~\eqref{eq:opt} is shown to be concave. Since the feasible solution set is convex a unique maximizer, called the optimal solution, exists.
\end{proof}

\subsection{Content Providers with Common Objects}
Here, we first assume there are only two content providers in the network and then consider the general case. Let $F_1$ and $F_2$ denote the sets of files served by content providers one and two, respectively. Also, let ${F_c = F_1 \cap F_2}$ denote the set of files served by both content providers. To avoid trivial cases, we assume ${0 < |F_1 \cap F_2| < \min{\{|F_1|, |F_2|\}}}$.

%We can for example consider Amazon Video~\cite{} and Netflix~\cite{} as two content providers with content that can be reached from both.

We have two conceivable cases for the files in $F_c$: 1)~each content provider needs to keep its own copy of the content, \eg\ due to security reasons, or 2)~one copy can be kept in cache to serve requests to either of the content providers.

The first case can be treated as if there is no common content between the two content providers, and hence the same approach as in~\eqref{eq:opt} yields the optimal solution.


For the second case, we argue, through the following theorem, that partitioning the cache into three slices as shown in Figure~2 maximizes the sum of the utilities. The first partition is for the set of common files between the two content providers $F_c = F_1 \cap F_2$. The other two partitions are for the remaining files of each of the two content providers.

\begin{figure}[h]
\centering
  	\includegraphics[scale=0.24]{partition_shared.png}
\caption{Partitioning cache for two content providers with common content.}
 %\vspace{-0.5cm}
    \label{fig:partition_shared}
\end{figure}

\begin{theorem}
With two content providers that serve some common content, the cache should be partitioned into three slices; one shared partition for the set of common files, and two other partitions, one for each content provider.
\end{theorem}
\begin{proof}
See Appendix~\ref{sec:proof_common}.
\end{proof}

We can now write the optimization problem for utility-driven resource allocation as follows:
\begin{align}
\label{eq:opt2}
\text{maximize} \quad &w_1 U_1(h_1) + w_2 U_2(h_2) \notag\\
\text{such that} \quad &C_1 + C_2 + C_3 \le C \\
& C_1, C_2, C_3 \ge 0, \notag
\end{align}
where the average hit rate $h_k, k=1,2$ is defined as
\begin{align*}
h_k &= \sum_{i\in F_k\char`\\ F_c}{\lambda_{ik}(1-e^{-\lambda_{ik}T_k})} \\
&\quad\quad + \sum_{i\in F_c}{\lambda_{ik}(1 - e^{-(\lambda_{i1}+\lambda_{i2})T_3})},
\end{align*}
where $T_3$ and $T_k$ are the unique solutions to the equations
\[\sum_{i\in F_c}{(1 - e^{-(\lambda_{i1}+\lambda_{i2})T_3})} = C_3,\]
and
\[\sum_{i\in F_k\char`\\ F_c}{(1 - e^{-\lambda_{ik}T_k})} = C_k, \quad k=1,2.\]

Based on the solution for the case of two content providers with common contents, and by induction one can see that for $K$ content providers with common files, its best to create a partition for each set of files that are served by a number of content providers. A procedure for creating the optimal set of partitions $\mathcal{P}$ with the files routed to each partition is given in Algorithm~\ref{alg:partition}. Algorithm~\ref{alg:partition} runs in $O(|F|^2)$ where $F$ denotes the set of all files served by all content providers. Here, we have assumed that the number of content providers is fixed. Note that the number of partitions can grow exponentially with the number of content providers.

\begin{algorithm}[t]
\caption{Partitioning a Cache serving $K$ content providers with possibility of common files among some content providers.}
\label{alg:partition}
\begin{algorithmic}[1]
	\Statex
		\State $F\gets F_1 \cup F_2 \cup \ldots \cup F_K$.
		\State $\mathcal{P}\gets \O$.
		\For{$f\in F$}
			\State $S_f\gets \{k:$ Content provider $k$ serves files $f\}$.
			\If{Exists $(V,S)\in P$ such that $S = S_f$}
				\State $V\gets V\cup \{f\}$.
			\Else
				\State $\mathcal{P}\gets \mathcal{P}\cup \{(\{f\}, S_f)\}$.
			\EndIf
		\EndFor
\end{algorithmic}
\end{algorithm}

Once the number of partitions $|\mathcal{P}|$ and the set of files corresponding to each partition is determined, the optimal partition size can be computed through the following optimization problem:
\begin{align}
\label{eq:opt3}
\text{maximize} \quad &\sum_k{w_k U_k(h_k)} \notag\\
\text{such that} \quad &\sum_{p=1}^{|\mathcal{P}|}{C_p} \le C \\
& C_p \ge 0,  \quad p=1, 2, \ldots, |\mathcal{P}|, \notag
\end{align}
where the average hit rate for each content provider is computed as
\[h_k = \sum_{p=1}^{|\mathcal{P}|}{\sum_{i\in V_p}{\lambda_{ik}(1 - e^{-\lambda_it_p})}},\]
where  $V_p$, denotes the set of files requested from partition $p$, and $\lambda_i\triangleq \sum_k{\lambda_{ik}}$ denotes the aggregate request rate for content $i$ through all content providers, and $t_p$ denotes the characteristic time of the partition serving content $p$.

\begin{theorem}
Resource allocation problem~\eqref{eq:opt3} has a unique optimal solution.
\end{theorem}
\begin{proof}
In Appendix~\ref{sec:proof_obj_shared}, we show that the optimization problem~\eqref{eq:opt3} has a concave objective function. Since the feasible solution set is convex, a unique maximizer exists.
\end{proof}

\subsection{Implications}


%\subsubsection{Sharing is Partitioning!}
\vspace*{1pt}
\noindent
{\bf Sharing is Partitioning!}
We have established -- with a formal proof in
Appendix~\ref{sec:proof_partition} -- that sharing a cache between two
content providers does not perform better than partitioning the cache
when the content providers have distinct sets of content objects. To understand better why that is the case we explain through the notion of cache characteristic time that sharing a cache is equivalent to partitioning it in a specific way.

Assume two content providers share an LRU cache of size $C$ that has characteristic time $T$. From the discussion in Section~\ref{sec:model}, we know that this assumption implies the following equation:
\[\sum_{k=1}^2{\sum_{i\in F_k}{(1-e^{-\lambda_{ik}T})}} = C.\]

However, we can also see that partitioning the cache into two
partition with sizes $C_1 = \sum_{i\in F_1}{(1-e^{-\lambda_{i1}T})}$
and $C_2 = \sum_{i\in F_2}{(1-e^{-\lambda_{i2}T})}$ achieves the same
utility values for the two content providers. Therefore, performance
of sharing the cache can be obtained by partitioning it according to
$C_1$ and $C_2$ as explained above.

%\subsubsection{Static Caching}
\vspace*{2pt}
\noindent
{\bf Cache Partitioning: Number of Slices, Management Complexity and
Static Caching.}
In our formulations and solutions of the multi-CP cache allocation problem via the
utility maximization framework (\eqref{eq:opt}) \& (\eqref{eq:opt3}),
cache is only partitioned and allocated per CP for a set of {\em distinct}content
objects owned by the CP; a cache slice is allocated and shared among
several CPs  only for a set of {\em common} content objects belonging
to these CPs. In other words, a CP with a set of distinct content
object, its cache slice is {\em not} further partitioned into smaller
slices for this CP. This is justified by cache management complexity
consideration, as further partitioning of the slice allocated for the
CP to be exclusively utilized by the same CP simply incurs additional
managment complexity. In addition,
Lemma~\ref{lemma:probabilistic-routing} in the Appendices shows that
by partitioning a cache slice into smaller slices and employing each
smaller slice to cache all content objects of the same CP via {\em
  probabistically content routing} is sub-optimal. As an alternative
to the CP-oriented cache allocation and partitioning approach, one
could adopt a per-object cache allocation and partitioning approach
(regardless of the CP or CPs which own the objects). Under such an
approach, it is not hard to show that the optimal {\em per-object} cache
allocation strategy that maximizes the overall cache hit rate is
equivalent to  the {\em static caching} policy~\cite{Liu98}:  the cache is only
allocated to the $K$ most popular objects among all content providers
that fill up the cache. Alternatively, such a solution can also be
obtained using the same CP-oriented, utility maximization cache
allocation framework where we replace the LRU cache replacement policy
with the static caching policy.


%\subsubsection{Utility Functions and Fairness}
\vspace*{2pt}
\noindent
{\bf Utility Functions and Fairness.}
Using different utility functions in the optimization formulations~\eqref{eq:opt} and~\eqref{eq:opt3} yield different partition sizes for the content providers. In this sense, each utility function defines a notion of fairness in allocating storage resources to different content providers. The family of $\beta$-fair utility functions expressed as
\[U_k(h_k) = \frac{h_k^{1-\beta}}{1-\beta},\]
unifies different notions of fairness in resource allocation~\cite{srikant13}. Some choices of $\beta$ lead to especially interesting utility functions. Table~\ref{tbl:util} gives a brief summary of these functions. We will use these functions in Section~\ref{sec:simulation} in understanding the effect of particular choices for utility functions, and in evaluating our proposed algorithms.

\begin{table}[]
%\centering
\caption{$\beta$-fair utility functions}
\hspace*{-0.5cm}
\begin{tabular}{ | c | c | c | c |}
\hline
$\beta$ & $\max{\sum_{k}{w_kU_k(h_k)}}$ & implication \\
\hline
  0 & $\max{\sum{w_k h_k}}$ & maximizing overall throughput \\
  1 & $\max{\sum{w_k \log{h_k}}}$ & proportional fairness \\
  2 & $\max{-\sum{w_k / h_k}}$ & minimize potential delay \\
  $\infty$ & $\max{\min{h_k}}$ & max-min fairness \\
\hline
\end{tabular}
\label{tbl:util}
\end{table}


==> proof_common.tex <==
\begin{proof}
It is known that with two content providers we have the following choices regarding how to utilize the cache: 1) no partitioning; 2) partitioning the cache into two fragments each dedicated to a provider; 3) partitioning the cache into three fragments with the third fragment serving common objects. In Theorem 2 we have shown that partitioning the cache into two fragments could improve the system performance as compared to no partitioning. We now show that partitioning the cache into three fragments could further improve the performance. Actually, we can imagine that there are four cache partitions where the cache is partitioned into two fragments each dedicated to a provider. Among the four partitions, two of them are serving the content set $F_1\backslash F_c$, $F_2\backslash F_c$, respectively, and the other two are serving the common set $F_c$. Now if we combine this two partitions serving the common set $F_c$ into one, then the hit rate of both content providers will increase as the hit rate for the files in common set $F_c$ are increased while the hit rate for the remaining files ($F_1\backslash F_c$ and $F_2\backslash F_c$) are kept unchanged. Therefore, we can see that partitioning the cache into three segments with one serving common files performs the best among the 3 choices. The optimal partitioning that maximizes system performance could be obtained by solving the optimization problem (2).
\end{proof}

==> proof_k_partitions.tex <==
\begin{proof}
First, suppose the cache should be partitioned into less than $K$ fragments. Then there must be some fragments that are shared by more than just one content provider. For each of these fragments, as the corresponding content providers are sharing the same characteristic time, we are able to find a partitioning where each provider is allocated to a dedicated fragment, and this partitioning provides the same request hit rate/probability as that without partitioning. We can then combine the fragments for the same content provider and this increases its request hit rate/probability. Therefore, we can see that partitioning the cache into $K$ fragments can provide better performance as compared to partitioning it into less number of fragments.

Now, suppose the cache should be partitioned into more than $K$ fragments. Then there must be some content providers to which more than one fragment are allocated. For each of these content providers, combining their dedicated fragments into one would improve their hit rate/probability. Therefore, the cache should be partitioned into no more than $K$ fragments.

Combining the above two, we can see that the cache should be partitioned into $K$ fragments.
\end{proof}

==> proof_obj.tex <==
\begin{proof}

\end{proof}

==> proof_partitioning_sharing.tex <==
\begin{proof}
Consider two content providers that serve the set of files $F_1$ and $F_2$, respectively, and access a cache of size $C$. Let $T$ denote the characteristic time of the cache when the cache is shared between the content providers. Based on the discussion in Section~\ref{sec:model}, we know that $T$ is the solution to the equation
%\[\sum_{i\in F_1\backslash F_c}{o(\lambda_{i1},T)} + \sum_{i\in F_c}{o(\lambda_{i1}+\lambda_{i2},T)}+\sum_{i\in F_2\backslash F_c}{o(\lambda_{i2},T)} = C.\]
\begin{align*}
&\sum_{i\in F_1\backslash F_c}{o(\lambda_{i1},T)} + \sum_{i\in F_c}{o(\lambda_{i1}+\lambda_{i2},T)} \\
&\qquad\qquad\qquad\qquad\qquad + \sum_{i\in F_2\backslash F_c}{o(\lambda_{i2},T)} = C.
\end{align*}

We can form partitions of size
\[C_1 = \sum_{i\in F_1\backslash F_c}{o(\lambda_{i1},T)},\]
\[C_2 = \sum_{i\in F_2\backslash F_c}{o(\lambda_{i1}+\lambda_{i2},T)},\]
and
\[C_s = \sum_{i\in F_c}{o(\lambda_{i2},T)},\]
to achieve the same utility values for the two content providers. 
Here, $C_1$ and $C_2$ denote the partition sizes dedicated to content providers one and two,
and $C_s$ denotes the size of the shared partition. Therefore, performance
of sharing the cache can be obtained by partitioning it to three slices as explained above.
\end{proof}



==> related_work-old.tex <==
\section{Related Work}
\subsection{Cache Partitioning}
Despite a plethora of research on the design and implementation of \emph{fair} and \emph{efficient} algorithms for differentiated bandwidth sharing in communication networks, little work has focused on the provision of multiple levels of service in web caches.
The available research has focused on designing biased replacement policies towards particular content classes~\cite{kelly99}, or using multiple levels of caches~\cite{feldman02}.
Hoteit et al~\cite{Hoteit15} have recently developed a game-theoretic cache allocation framework. 
Their approach requires the content providers to report the true demands from their content access.
Researchers in~\cite{ko03} and~\cite{lu04} were first to propose differentiated caching services via cache partitioning. Their techniques, however, either require additional controllers for fairness, or make inefficient use of the cache storage.

\subsection{Network Utility Maximization}
Utility functions have been widely used in modeling computer networks, from stability analysis of queues to the study of fairness in network resource allocation; see~\cite{srikant13, neely10} and references therein. Kelly~\cite{kelly97} was the first to suggest that the problem of rate allocation can be formulated as one of achieving maximum
aggregate utility for users, and described how network-wide optimal rate allocation could be achieved by having individual users control their transmission rates.
The seminal work by Kelly~\etal~\cite{kelly98} presents the first mathematical model and analysis of the behavior of congestion control algorithms for general topology networks.
Since then, there has been extensive research in generalizing and applying Kelly's \emph{Network Utility Maximization} framework to model and analyze various network protocols and architectures. This framework has been used to study problems such as network routing~\cite{Kleinberg99}, throughput maximization~\cite{eryilmaz07}, dynamic power allocation~\cite{neely03} and scheduling in energy harvesting networks~\cite{huang13}, among many others.

To the best of our knowledge, this paper is the first attempt in design and modeling cache partitioning for web contents built upon the utility maximization framework.

==> simulation_old.tex <==
\section{Evaluation}
\label{sec:simulation}
In this section, we perform numerical simulations, first to understand the efficacy of cache partitioning on the utility observed by content providers, and second to evaluate the performance of our proposed online algorithms.

For our base case, we consider a cache with capacity for $C=10^4$ files and two content providers with $N_1 = 10^4$ and $N_2 = 2\times 10^4$ content files. File popularities for the two content providers follow Zipf distributions with parameters $\alpha_1 = 0.6$ and $\alpha_2 = 0.8$, respectively. Requests for the files from the two content providers arrive as Poisson processes with aggregate rates $\lambda_1 = 15$ and $\lambda_2=10$. The utilities of the two content providers are expressed as $U_1(h_1) = \log{h_1}$ and $U_2(h_2) = h_2$. Moreover, we assume the two content providers are equally important to the service provider, \ie\ $w_1 = w_2 = 1$. We will evaluate the effect of these parameters on the optimal partitioning of the cache.

We further consider two scenarios here. In the first scenario, the two content providers serve completely separate files. In the second scenario, files ${f=1:3:10000}$, are served by both of the providers. For each scenario the appropriate optimization formulation is chosen.

\subsection{Cache Partitioning}
To understand the efficacy of cache partitioning, we first look at solutions computed by the optimization problems~\eqref{eq:opt} and~\eqref{eq:opt3}. Figure~\ref{fig:up} shows the gain in total utility through partitioning the cache, by comparing the utility obtained by sharing the cache between the content providers and the utility obtained by partitioning the cache. In this example, up to $10\%$ increase is observed in total utility when content providers serve distinct sets of files, while around $30\%$ increase in total utility is seen when some content is served by both of the content providers.

\begin{figure}[]
\centering
 \begin{subfigure}[b]{0.5\linewidth}
  	\centering\includegraphics[scale=0.3]{utility_partition.eps} % up
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.5\linewidth}
  	\centering\includegraphics[scale=0.3]{utility_partition_shared.eps}
  	\caption{}
 \end{subfigure}%
%\vspace{-0.25cm}
 \caption{Efficacy of cache partitioning when (a) content providers serving distinct files, (b) some content is served by both content providers.}
    \centering\label{fig:up}
\end{figure}

We next look at the effect of various parameters on cache partitioning. For each parameter, we show the effect on the hit rates and partition sizes for the two scenarios when content providers serve distinct files and when some content is served by both. Figures~\ref{fig:bwlama}(a)-(d) show the effect of changing the weight parameter for the first content provider $w_1$. As it is expected, by increasing the weight $w_1$, content provider one gets a larger share of the cache, and hence a higher hit rate.

Figures~\ref{fig:bwlama}(e)-(h) show the effect of changing the aggregate arrival rate for the first content provider $\lambda_1$. In this case, no change in observed in the partition sizes. This is because the first content provider uses the $\log$ utility function, and it is easy to see that the derivative ${U'_1(h_1)\partial h_1/\partial C_p}$ does not depend on the aggregate rate. In our example, changing the aggregate request rate for the second content provider with $U_2(h_2) = h_2$ would result in different partition sizes.

Figures~\ref{fig:bwlama}(i)-(l) show how resource allocation for each content provider changes 
as the skewness parameter $\alpha_1$ from the Zipfian content popularity distribution changes for the first content provider. As file popularities get more skewed, a smaller number of files make up for a big portion of the aggregate request rate. Therefore, a smaller partition size can still yield a higher hit rate. Hence, dedicated partition size for content provider one decreases as $\alpha_1$ increases.

In Figures~\ref{fig:bwlama}(m)-(p), we use change the utility function of the first content provider by using the $\beta$-fair utility functions with different values of $\beta$. As the value of $\beta_1$ increases the first content provider consumes less resources from the cache and its hit rate decreases.

\begin{figure*}[t]
\centering
\begin{subfigure}[b]{\linewidth}
  	\centering\includegraphics[scale=0.5]{legend.png}
 \end{subfigure}
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_WW_lam_a_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_WW_lam_a_partitions.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_WW_lam_a_shared_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_WW_lam_a_shared_partitions.eps}
  	\caption{}
 \end{subfigure}
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_LAMLAM_a_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_LAMLAM_a_partitions.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_LAMLAM_a_shared_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_LAMLAM_a_shared_partitions.eps}
  	\caption{}
 \end{subfigure}
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_lam_AA_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_lam_AA_partitions.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_lam_AA_shared_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{b_w_lam_AA_shared_partitions.eps}
  	\caption{}
 \end{subfigure}
  \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{BB_w_lam_a_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{BB_w_lam_a_partitions.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{BB_w_lam_a_shared_hitrates.eps}
  	\caption{}
 \end{subfigure}%
 \begin{subfigure}[b]{0.25\linewidth}
  	\centering\includegraphics[scale=0.3]{BB_w_lam_a_shared_partitions.eps}
  	\caption{}
 \end{subfigure}
%\vspace{-0.25cm}
 \caption{Effect of the parameters on the partition sizes and hit rates.}
    \centering\label{fig:bwlama}
\end{figure*}

%\begin{figure}[]
%\centering
% \begin{subfigure}[b]{0.5\linewidth}
%  	\centering\includegraphics[scale=0.3]{ubeta_hit_rate.eps}
% \end{subfigure}%
% \begin{subfigure}[b]{0.5\linewidth}
%  	\centering\includegraphics[scale=0.3]{ubeta_partition_size.eps}
% \end{subfigure}%
%%\vspace{-0.25cm}
% \caption{Utility. }
%    \centering\label{fig:ubeta}
%\end{figure}

\subsection{Online Algorithms}
Here, we evaluate the  online algorithms explained in Section~\ref{sec:online} through numerical simulations. Requests are generated according to the parameters described in the beginning of the section, and the service provider adjusts partition sizes based on the number of request hits between iterations. The service provider is assumed to know the utility functions of the content providers. The utility function of the first content provider is fixed to be $U_1(h_1) = \log{h_1}$. We consider three utility functions for the second content provider, namely $U_2(h_2) = h_2$, $U_2(h_2) = \log{h_2}$ and $U_2(h_2) = -1/h_2$.

\begin{figure*}[t]
\centering
 \begin{subfigure}[b]{0.33\linewidth}
  	\centering\includegraphics[scale=0.4]{1_h.eps}
  	\caption{$U_2(h_2) = h_2$.}
 \end{subfigure}%
 \begin{subfigure}[b]{0.33\linewidth}
  	\centering\includegraphics[scale=0.4]{1_log_h.eps}
  	\caption{$U_2(h_2) = \log{h_2}$.}
 \end{subfigure}%
 \begin{subfigure}[b]{0.33\linewidth}
  	\centering\includegraphics[scale=0.4]{1_inv_h.eps}
  	\caption{$U_2(h_2) = -1/h_2$.}
 \end{subfigure}%
%\vspace{-0.25cm}
 \caption{Convergence of the online algorithm when content providers serve distinct files. $U_1(h_1) = \log{h_1}$.}
    \centering\label{fig:online}
\end{figure*}

We first consider the case where content providers serve distinct files. We initially partition the cache into two equal segments $C_1 = C_2 = 5000$ and use Algorithm~\ref{alg:online} to obtain the optimal partition sizes. Figure~\ref{fig:online} shows how the partition sizes for the two content providers change at each iteration of the algorithm and converge to the optimal values computed from~\eqref{eq:opt}, marked with dashed lines. Figure~\ref{fig:online_utility} shows how total utility increases at each iteration.

\begin{figure}[h]
\centering
  	\includegraphics[scale=0.4]{online_utility.eps}
%\vspace{-0.3cm}
  \caption{Total utility increases and stabilizes.}
    \label{fig:online_utility}
\end{figure}

Next, we consider the case where some content is served by both of the content providers. We start by partitioning the cache as $C_1=C_2 = 4000$ and $C_3=2000$, and use Algorithm~\ref{alg:online_shared} to obtain the optimal partitioning. Figure~\ref{fig:online_shared} shows the changes in the three partitions as the algorithm converges to a stable point. For each partition the optimal size computed by~\ref{eq:opt2} is shown by dashed lines.

\begin{figure*}[t]
\centering
 \begin{subfigure}[b]{0.33\linewidth}
  	\centering\includegraphics[scale=0.4]{online_shared_1_0.eps}
  	\caption{$U_2(h_2) = h_2$.}
 \end{subfigure}%
 \begin{subfigure}[b]{0.33\linewidth}
  	\centering\includegraphics[scale=0.4]{online_shared_1_1.eps}
  	\caption{$U_2(h_2) = \log{h_2}$.}
 \end{subfigure}%
 \begin{subfigure}[b]{0.33\linewidth}
  	\centering\includegraphics[scale=0.4]{online_shared_1_2.eps}
  	\caption{$U_2(h_2) = -1/h_2$.}
 \end{subfigure}%
%\vspace{-0.25cm}
 \caption{Convergence of the online algorithm when some content is served by both content providers. $U_1(h_1) = \log{h_1}$.}
    \centering\label{fig:online_shared}
\end{figure*}
